XScale-NVS: Cross-Scale Novel View Synthesis with Hash Featurized Manifold

We propose XScale-NVS for high-fidelity cross-scale novel view synthesis of real-world large-scale scenes. Existing representations based on explicit surface suffer from discretization resolution or UV distortion, while implicit volumetric representations lack scalability for large scenes due to the dispersed weight distribution and surface ambiguity. In light of the above challenges, we introduce hash featurized manifold, a novel hash-based featurization coupled with a deferred neural rendering framework. This approach fully unlocks the expressivity of the representation by explicitly concentrating the hash entries on the 2D manifold, thus effectively representing highly detailed contents independent of the discretization resolution. We also introduce a novel dataset, namely GigaNVS, to benchmark cross-scale, high-resolution novel view synthesis of realworld large-scale scenes. Our method significantly outperforms competing baselines on various real-world scenes, yielding an average LPIPS that is 40% lower than prior state-of-the-art on the challenging GigaNVS benchmark. Please see our project page at: xscalenvs.github.io.

==> elements/figures/feat_resol.tex <==
\begin{figure}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.5}
    \newcommand{\figw}{0.45} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/method_pics/feat_resol.png}
    \vspace{-1em}
    \caption{Illustration of the featuremetric resolution issue. }
    \hfill
    \vspace{-1em}
    \label{fig:feat_resol}
\end{figure}

==> elements/figures/qualitative_6k.tex <==
\begin{figure*}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{1.0} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/qualitative_6k.jpg}
    \vspace{-2.2em}
    \caption{Qualitative results of 5K-resolution novel view synthesis on the \texttt{GigaNVS} dataset. Our method fully exploits the input resolution and demonstrates strong scalability towards high-resolution neural rendering. Please zoom-in to see the high-resolution details.}
    \hfill
    % \vspace{-1.0em}
    \label{fig:qualitative_6k}
\end{figure*}

==> elements/figures/qualitative_md.tex <==
\begin{figure}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{0.48} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    % \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/ablation_md.jpg}
    \vspace{-2.5em}
    \caption{Qualitative comparisons of novel view synthesis with different levels of featurization enhancements. Sharp details can be effectively recovered with surface multisampling (M) and manifold deformation (D).}
    \hfill
    \vspace{-1.0em}
    \label{fig:ablation_md}
\end{figure}

==> elements/figures/qualitative_mesh.tex <==
\begin{figure*}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{1.0} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/mesh_supp.jpg}
    \vspace{-2.2em}
    \caption{Qualitative results with different mesh resolutions on the Sandie Spring scene of \texttt{GigaNVS} dataset, where our novel view RGB renderings and the corresponding mesh normals are visualized. The first two rows are macro-scale renderings from a distance and the last two rows are micro-scale renderings at the close-up. Our method robustly recovers scene contents at drastically different scales when down-sampling the mesh to lower resolutions.}
    \hfill
    \vspace{-1.5em}
    \label{fig:qualitative_mesh}
\end{figure*}

==> elements/figures/qualitative_relit.tex <==
\begin{figure*}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{1.0} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    % \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/qualitative_relit.jpg}
    \vspace{-2.0em}
    \caption{Qualitative relighting results on the TW-Pavilion (Day) scene when varying the lighting embedding.}
    \hfill
    \vspace{-1.5em}
    \label{fig:qualitative_relit}
\end{figure*}

==> elements/figures/qualitative_resol.tex <==
\begin{figure}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{0.48} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    % \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/qualitative_resol.jpg}
    \vspace{-1.5em}
    \caption{Quantitative and qualitative evaluations with different featuremetric resolutions (2$^{10}$ $\sim$ 2$^{13}$).}
    \hfill
    \vspace{-2.2em}
    \label{fig:qualitative_resol}
\end{figure}

==> elements/figures/qualitative_tanks.tex <==
\begin{figure*}[htbp]
    \centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{1.0} % can bigger than 1
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/qualitative_tanks.pdf}
\hfill
\vspace{-1.5em}
\centerline{\footnotesize{\hspace{-1.5em}
    (a) 3D Gaussian Splatting~\cite{kerbl20233d}\hspace{2.0em}(b) Neuralangelo~\cite{li2023neuralangelo}\hspace{5.0em}
    (c) iNGP~\cite{muller2022instant}\hspace{8.0em}(d) \textbf{Ours}\hspace{6.0em}
    (e) Ground Truth Image}}
\vspace{-1.5em}
\caption{Visual comparisons on the Tanks\&Temples dataset~\cite{knapitsch2017tanks}. Our method excels at recovering local intricate details yet generally performs on par with state-of-the-art neural rendering methods~\cite{kerbl20233d, muller2022instant, li2023neuralangelo} on small-scale scenes.}
\vspace{-0.5em}
\label{fig:qualitative_tanks}
\end{figure*}

==> elements/figures/qualitative_teaser.tex <==
\begin{figure*}[htbp]
% \begin{figure*}[h|]
    \centering
    \newcommand{\colw}{0.19}
    \newcommand{\figw}{1.0} % can bigger than 1 
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/method_pics/qualitative_teaser.jpg}
    \hfill
    \vspace{-1.5em}
    \centerline{\normalsize{\hspace{-4.0em}
    (a) Meta Representation~\cite{10274871}\hspace{0.7em}(b) 3D Gaussian Splatting~\cite{kerbl20233d}\hspace{2.0em}(c) Neuralangelo~\cite{li2023neuralangelo}\hspace{6.0em}(d) \textbf{Ours}}}
\vspace{-1.5em}
\caption{We propose hash featurized manifold for deferred neural rendering of large-scale scenes with cross-scale contents. Compared to the recent advances in neural rendering~\cite{10274871, kerbl20233d, li2023neuralangelo}, our method synthesizes novel views with unprecedented levels of realism. Please zoom in to see the high-quality details. }
\vspace{-1em}
\label{fig:qualitative_teaser}
\end{figure*}

==> elements/figures/qualitative_twg_mesh.tex <==
\begin{figure*}[htbp]
    %\centering
    %\centering
    \newcommand{\colw}{0.2}
    \newcommand{\figw}{1.0} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    % \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/experiment_pics/mesh_supp_twg.jpg}
    \vspace{-2.2em}
    \caption{Qualitative results with different mesh resolutions on the TW-Pavilion (Day) scene of \texttt{GigaNVS} dataset. First row: our novel view RGB renderings; Second row: the corresponding rendered normals of the input mesh. }
    \hfill
    \vspace{-1.5em}
    \label{fig:qualitative_mesh_twg}
\end{figure*}

==> elements/figures/vol_weight.tex <==
\begin{figure}[htb]
    %\centering
    %\centering
    \newcommand{\colw}{0.5}
    \newcommand{\figw}{0.48} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    \vspace{-0.5em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/method_pics/vol_weight.jpg}
    \vspace{-2em}
    \caption{Visualization of the volume rendering weight distributions of Neuralangelo~\cite{li2023neuralangelo}. The middle image is the final RGB rendering. In each surrounding sub-figure, we plot the weight $w(t)$ for each individual sample at certain normalized distance $t$ traced from one of the labeled pixels. The red vertical lines denote the surface locations calculated by mesh rasterization. For brevity, we only show important samples near the surface. 
    % and the horizontal axis $t$ denotes the normalized ray distance when the entire scene is transformed into a unit bounding sphere.
    }
    \hfill
    \vspace{-1em}
    \label{fig:vol_weight}
\end{figure}

==> elements/figures/zip.tex <==
\begin{figure}[H]
    %\centering
    %\centering
    \newcommand{\colw}{0.5}
    \newcommand{\figw}{0.3} % can bigger than 1
    %\begin{minipage}{\colw\linewidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{elements/figures/method_pics/zip.png}
    \vspace{-0.5em}
    \caption{Illustration of the proposed spatial multisampling and manifold displacement.
    \guangyu{embedd this fig into the pipeline figure.}}
    \hfill
    \vspace{-2em}
    \label{fig:zip}
\end{figure}

==> elements/tables/tab_mesh_supp_twg.tex <==
\begin{table}[htbp]
\scriptsize
\setlength{\tabcolsep}{1.3mm}{
\footnotesize
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c}{Method} & \#Primitives & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\ \hline
Ours & 10M & {23.02} & {0.786} & {0.113} \\ 
Ours & 5M & {22.94} & {0.785} & {0.112} \\
Ours & 2M & {22.87} & {0.783} & {0.112} \\ 
Ours & 1M & {22.84} & {0.782} & {0.114} \\
Ours & 0.5M & {22.44} & {0.767} & {0.125} \\
Ours & 0.2M & {22.07} & {0.749} & {0.140} \\
% 0.1M & {20.72} & {0.674} & {0.196} \\
\hline
3D Gaussian Splatting~\cite{kerbl20233d} & 3M & {21.52} & {0.752} & {0.225} \\
\hline
\end{tabular}
}
\vspace{-1.0em}
\caption{Mesh resolution ablation on the TW-Pavilion (Day) scene.}
\vspace{-1.0em}
\label{tab:ablation_mesh_twg}
\end{table}

==> elements/tables/tab_tanks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\footnotesize
\setlength{\tabcolsep}{0.55mm}{
% \caption{Quantitative comparisons at 1K (989$\times$ 1320) resolution on GigaNVS dataset. The proposed hash featurized manifold outperforms state-of-the-art approaches on all evaluation metrics.}
% \vspace{-1em}
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\tabincell{c}{Scene}} & \multicolumn{3}{c|}{Meta representation\cite{10274871}} & \multicolumn{3}{c|}{3D Gaussian Splatting\cite{kerbl20233d}} & \multicolumn{3}{c|}{Neuralangelo\cite{li2023neuralangelo}} & \multicolumn{3}{c|}{iNGP\cite{muller2022instant}} & \multicolumn{3}{c}{\textbf{Ours}} \\ \cline{2-16}
{} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$\\ \hline
Family & 27.92 & 0.913 & \cellcolor{Third}0.035 & \cellcolor{First}{28.54} & \cellcolor{Second}0.920 & \cellcolor{Third}0.035 & 28.02 & \cellcolor{First}{0.922} & \cellcolor{Second}0.033 & \cellcolor{Second}{28.49} & \cellcolor{Third}{0.919} & {0.036} & \cellcolor{Third}{28.15} & {0.915} & \cellcolor{First}{0.032} \\
Francis & \cellcolor{Third}33.11 & \cellcolor{Third}0.958 & \cellcolor{Second}0.048 & \cellcolor{First}{35.77} & \cellcolor{Second}0.969 & \cellcolor{Third}0.050 & 30.54 & 0.951 & 0.056 & {31.85} & {0.950} & {0.067} & \cellcolor{Second}35.32 & \cellcolor{First}{0.973} & \cellcolor{First}{0.024} \\
Horse & \cellcolor{Second}35.22 & \cellcolor{Third}0.979 & 0.027 & 34.88 & \cellcolor{First}{0.986} & \cellcolor{Second}0.017 & 34.62 & \cellcolor{Second}0.984 & \cellcolor{First}{0.016} & \cellcolor{Third}{35.16} & \cellcolor{Second}{0.984} & \cellcolor{Third}{0.018} & \cellcolor{First}{36.07} & \cellcolor{Second}0.984 & \cellcolor{Second}0.017 \\
M60 & 27.36 & 0.891 & 0.153 & \cellcolor{First}{29.41} & \cellcolor{First}{0.918} & \cellcolor{Third}0.133 & 27.03 & 0.886 & 0.154 & \cellcolor{Second}{28.82} & \cellcolor{Second}{0.907} & \cellcolor{Second}{0.132} & \cellcolor{Third}28.07 & \cellcolor{Third}0.899 & \cellcolor{First}{0.115} \\
Lighthouse & 23.92 & 0.811 & 0.201 & 22.49 & 0.825 & 0.207 & \cellcolor{Third}23.96 & \cellcolor{Third}{0.836} & \cellcolor{Third}0.191 & \cellcolor{Second}{24.47} & \cellcolor{Second}{0.842} & \cellcolor{Second}{0.187} & \cellcolor{First}{26.47} & \cellcolor{First}{0.866} & \cellcolor{First}{0.127} \\
Panther & \cellcolor{Third}28.57 & 0.889 & 0.162 & 26.83 & 0.869 & 0.210 & 27.87 & \cellcolor{Third}0.901 & \cellcolor{Third}0.155 & \cellcolor{First}{29.70} & \cellcolor{First}{0.908} & \cellcolor{Second}{0.146} & \cellcolor{Second}{29.05} & \cellcolor{Second}{0.903} & \cellcolor{First}{0.112} \\
Train & 22.12 & 0.803 & 0.207 & \cellcolor{Second}22.44 & \cellcolor{Second}0.834 & 0.206 & 19.85 & 0.806 & \cellcolor{Third}0.195 & \cellcolor{Third}{22.21} & \cellcolor{Third}{0.826} & \cellcolor{Second}{0.184} & \cellcolor{First}{24.50} & \cellcolor{First}{0.863} & \cellcolor{First}{0.124} \\ \hline
Mean & 28.32 & 0.892 & 0.119 & \cellcolor{Third}28.62 & \cellcolor{Third}0.903 & 0.123 & 27.41 & 0.898 & \cellcolor{Third}0.114 & \cellcolor{Second}{28.67} & \cellcolor{Second}{0.905} & \cellcolor{Second}{0.110} & \cellcolor{First}29.66 & \cellcolor{First}0.914 & \cellcolor{First}0.079 \\ \hline
\end{tabular}
}
\vspace{-1em}
\caption{Quantitative comparisons on seven scenes from the Tanks\&Temples dataset. 
% Our method also outperforms state-of-the-art approaches on small-scale scenes.
}
\label{tab:tanks}
\vspace{1.0em}
\end{table*}
